Electronic layer decoupling driven by density-wave order in La$_4$Ni$_3$O$_{10}$

We probe the density-wave transition of the trilayer nickelate La$_4$Ni$_3$O$_{10}$ with polarization-resolved infrared spectroscopy. The low-energy electrodynamics is strongly anisotropic, with metallic in-plane and insulating out-of-plane character. In the ordered phase, the anisotropy grows more than an order of magnitude as the out-of-plane conductivity is sharply suppressed. We interpret this enhancement as an effective electronic decoupling of the Ni-O layers, driven by a spin-density-wave-induced redistribution of Ni-$d_{z^2}$ occupation within the trilayers. This electronic response is accompanied by clear shifts and splittings of the out-of-plane phonons, compatible with a density-wave instability of electronic origin.

==> latexmkrc <==
# Use pound symbols to comment lines that you do not want to run

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

# main text
#$pdflatex = "latexdiff OLD.tex main.tex  > main-d.tex; pdflatex %O  main-d"

# supp
#$pdflatex = "latexdiff supp_old.tex supp.tex  > main-d.tex; pdflatex %O  main-d"
